ELFS: Label-Free Coreset Selection with Proxy Training Dynamics

High-quality human-annotated data is crucial for modern deep learning pipelines, yet the human annotation process is both costly and time-consuming. Given a constrained human labeling budget, selecting an informative and representative data subset for labeling can significantly reduce human annotation effort. Well-performing state-of-the-art (SOTA) coreset selection methods require ground truth labels over the whole dataset, failing to reduce the human labeling burden. Meanwhile, SOTA label-free coreset selection methods deliver inferior performance due to poor geometry-based difficulty scores. In this paper, we introduce ELFS (Effective Label-Free Coreset Selection), a novel label-free coreset selection method. ELFS significantly improves label-free coreset selection by addressing two challenges: 1) ELFS utilizes deep clustering to estimate training dynamics-based data difficulty scores without ground truth labels; 2) Pseudo-labels introduce a distribution shift in the data difficulty scores, and we propose a simple but effective double-end pruning method to mitigate bias on calculated scores. We evaluate ELFS on four vision benchmarks and show that, given the same vision encoder, ELFS consistently outperforms SOTA label-free baselines. For instance, when using SwAV as the encoder, ELFS outperforms D2 by up to 10.2% in accuracy on ImageNet-1K. We make our code publicly available on GitHub.

==> tables/ccs_label_free_compare.tex <==
\begin{table}[ht!]
    \centering
    \caption{Performance comparison of label-free CCS, supervised CCS, \method, and label-free D2 on CIFAR100, using forgetting scores derived from DINO pseudo-label training.}
    \label{tab:ccs_label_free}
    \resizebox{0.55\textwidth}{!}{  
    \begin{tabular}{lccccc}
        \toprule
        Pruning rate & 30\% & 50\% & 70\% & 80\% & 90\% \\
        \midrule
        D2 (Best Label-Free) & 75.3 & 71.3 & 66.0 & 56.2 & 42.1 \\
        CCS (Pseudo Label)& 75.5 & 72.9 & 67.2 & 60.9 & 51.8 \\
        \method & 76.8 & 74.0 & 68.4 & 61.9 & 54.9 \\
        \midrule
        CCS (Supervised) & 77.1 & 74.5 & 68.9 & 64.0 & 56.0\\
        \bottomrule
    \end{tabular}
    }
    
    
\end{table}



==> tables/imagenet_results.tex <==
\begin{table}[ht!]
    \centering
    \caption{Performance evaluation varing pruning rates for ImageNet-1K dataset.}
    \label{tab:imagenet_results}
    \resizebox{0.52\textwidth}{!}{%
    \begin{tabular}{@{}lccccccc@{}}
        \toprule
        Pruning Rate   & 0\% & 30\% & 50\% & 70\% & 80\% & 90\% \\
        \midrule
        Random & 73.1 & 72.2 & 70.3 & 66.7 & 62.5 & 52.3 \\
        Prototypicality~\citep{prototypicality} & - & 70.9 & 60.8 & 54.6 & 41.9 & 30.6 \\
        Badge~\citep{ash2019deep} & - & 71.7 & 70.4 & 65.8 & 61.7 & 53.4 \\
        D2 (label free)~\citep{maharana2023d2} & - & 72.3 & 65.6 & 55.6 & 50.8 & 43.2 \\
        \cmidrule(lr){1-7} 
        \method (DINO) & - & \textbf{73.5} & \textbf{71.8} & \textbf{67.2} & \textbf{63.4} & \textbf{54.9} \\
        \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/model_ablation.tex <==
\begin{table}[ht!]
    \vspace{0.2cm}
    \centering
    \caption{Performance evaluation of distance-based baseline using different pretrained models embeddings on CIFAR10. }
    \resizebox{0.75\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        & \multicolumn{5}{c}{DINO} & \multicolumn{5}{c}{SwAv} \\
        \cmidrule(lr){2-6} \cmidrule(lr){7-11}
        Pruning Rate & 30\% & 50\% & 70\% & 80\% & 90\% & 30\% & 50\% & 70\% & 80\% & 90\% \\
        \midrule
        Prototypicality & 94.9 & 93.8 & 86.6 & 75.7 & 42.6 & 94.7 & 92.9 & 90.1 & 84.2 & 70.9 \\
        Label-free D2 & 94.2 & 93.1 & 91.5 & 88.2 & 82.8 & 94.3 & 93.8 & 91.6 & 85.1 & 71.4 \\
        \midrule
        \method &  \textbf{95.5} & \textbf{95.2} & \textbf{93.2} & \textbf{90.7} & \textbf{87.3} &  \textbf{95.0} & \textbf{94.3} & \textbf{91.8} & \textbf{89.8} & \textbf{82.5}  \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:model_ablation}
    \vspace{0.2cm}
\end{table}


==> tables/overheads.tex <==
\begin{table}[ht!]
    \centering
    \vspace{0.2cm}
    \caption{Computational Overhead for \method on various datasets, measured from the runtime on NVIDIA 2080Ti GPUs, on a Linux server with 128G GPU VRAM.}
    \resizebox{0.8\textwidth}{!}{%
    \begin{tabular}{lcccccc}
        \toprule
        {Dataset}
        & CIFAR10 & CIFAR100 & STL10 & CINIC-10 & ImageNet-1K \\
        \midrule
        \textbf{Pseudo-Label Generation} & & & & & \\
        \quad Embedding and K-NN & 2 min & 2 min & 2 min & 14 min & 4 hour 50 min \\
        \quad Clustering Head Training & 41 min & 41 min & 12 min & 4 hours 46 min & 34 hours \\
        \midrule
        \textbf{Data Difficulty Calculation} & & & & & \\
        \quad Training Dynamic Collection & 65 min & 65 min & 50 min & 80 min & 31 hours \\
        \quad Data Difficulty Calculation & 1 min & 1 min & 1 min & 2 min & 40 min \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:overheads}
    \vspace{0.2cm}
\end{table}

